How angry are your customers? Sentiment analysis of support tickets that escalate

Software support ticket escalations can be an extremely costly burden for software organizations all over the world. Consequently, there exists an interest in researching how to better enable support analysts to handle such escalations. In order to do so, we need to develop tools to reliably predict if, and when, a support ticket becomes a candidate for escalation. This paper explores the use of sentiment analysis tools on customer-support analyst conversations to find indicators of when a particular support ticket may be escalated. The results of this research indicate a considerable difference in the sentiment between escalated support tickets and non-escalated support tickets. Thus, this preliminary research provides us with the necessary information to further investigate how we can reliably predict support ticket escalations, and subsequently to provide insight to support analysts to better enable them to handle support tickets that may be escalated.

==> sections/machine_learning.tex <==
\section{Machine Learning}

To address RQ3, the emotion and tendency data was fed into ML models, the results of which are reported in this section. In addition to the ML work, however, three incremental datasets were built to identify if the models would perform better or worse given less --- but more specific --- data to learn and predict against.

\subsection{Incremental Datasets}



When using historical data with multiple time-based data points per unit of analysis, it is common to use all available data when building and testing a predictive model --- which for our analysis means using all emails up until the escalation occurred; however, that choice means predicting against data available right before the critical event, when it may be beneficial to ask how a model performs when it has been fed less than all available data. In our live system, waiting until the last possible moment to predict whether an item will escalate is too late, as it leaves support analysts no time to proactively work towards preventing the escalation.

If all emails of a support ticket are used to calculate the mean and Tendency, then the analysis is considered to have been applied to the \textit{100\% set}. If the first three quarters of all available emails are used in calculating Tendency, then the analysis applied is to the \textit{75\% set}. The first half of the emails is considered to be the \textit{50\% set}, and the first quarter is considered to be the \textit{25\% set}. 

For this research, the ML models were always trained using the 100\% sets, and then tested using all four sets separately. The reason for testing using all four sets (separately) is to understand how the models would have performed at different stages of the incoming data on these support tickets, if these models would have been running in real time. Testing on the 100\% set is conceptually asking how the ML models perform against data right up until the escalation event. By testing on the other sets, the results reflect how the ML models perform when only given the first 25\%, 50\%, and 75\% of the data, which conceptually allows an understanding of model performance at different stages of live support tickets.

The reason for training on the 100\% sets is because training on the smaller sets implies that some information is known about the test data that simply cannot be known at test time if these models are used against live data, which would give the models an unfair advantage for this analysis. For example, it may seem intuitive to train on the 25\% set when testing with the 25\% set, however, when working with live data, it will not be known how close to an escalation each support ticket is (or even which of these support tickets will escalate at all).

\subsection{Machine Learning Results}







==> sections/methodology.tex <==
\section{Methodology}
.
\\- data collection
\\- manual annotation
\\- normality testing
\\- difference testing
\\- machine learning
\\- stages of machine learning

To address our research questions, difference testing was applied to the data comparing Escalation and non-Escalation situations, and machine learning algorithms were utilized to test the performance of the data towards predicting Escalations.


Due to the state of the data, 





